Phase-resolved spectroscopy of a quasi-periodic oscillation in the black hole X-ray binary GRS 1915+105 with NICER and NuSTAR

Quasi-periodic oscillations (QPOs) are often present in the X-ray flux from accreting stellar-mass black holes (BHs). If they are due to relativistic (Lense-Thirring) precession of an inner accretion flow which is misaligned with the disc, the iron emission line caused by irradiation of the disc by the inner flow will rock systematically between red and blue shifted during each QPO cycle. Here we conduct phase-resolved spectroscopy of a $\sim2.2$ Hz type-C QPO from the BH X-ray binary GRS 1915+105, observed simultaneously with NICER and NuSTAR. We apply a tomographic model in order to constrain the QPO phase-dependent illumination profile of the disc. We detect the predicted QPO phase-dependent shifts of the iron line centroid energy, with our best fit featuring an asymmetric illumination profile ($>2{\sigma}$ confidence). The observed line energy shifts can alternatively be explained by the spiral density waves of the accretion-ejection instability model. However we additionally measure a significant ($>3{\sigma}$) modulation in reflection fraction, strongly favouring a geometric QPO origin. We infer that the disc is misaligned with previously observed jet ejections, which is consistent with the model of a truncated disc with an inner precessing hot flow. However our inferred disc inner radius is small ($r_\text{in}{\sim} 1.4 GM/c^2$). For this disc inner radius, Lense-Thirring precession cannot reproduce the observed QPO frequency. In fact, this disc inner radius is incompatible with the predictions of all well-studied QPO models in the literature.

==> Table_data/PRS/phase_diff.tex <==
	\begin{tabular}{lccr} % four columns, alignment for each
		\hline
		Mission & $\psi / \pi$ \\
		\hline
		NuSTAR & $0.21 \pm 0.02$ \\
		NICER & $0.123 \pm 0.006$ \\
		\hline
	\end{tabular}

==> Table_data/auto_temp/ftest_table.tex <==
\begin{tabular}{lrrr}
\toprule
Pars fixed to 0                                                                &	DOF  &	$\chi^2$ &	$\sigma$ \\ 
\midrule
None                                                                           &	3179 &	3374.61  &	N/A \\      
$A_1$, $\Phi_1$                                                                &	3181 &	3381.44  &	2.05 \\     
$A_2$, $\Phi_2$                                                                &	3181 &	3384.07  &	2.52 \\     
$A_1$, $A_2$, $\Phi_1$, $\Phi_2$                                               &	3183 &	3384.14  &	1.87 \\     
$A_{1\Gamma}$, $\phi_{1\Gamma}$, $A_{2\Gamma}$, $\phi_{2\Gamma}$               &	3183 &	3389.46  &	2.68 \\     
$A_{1e}$, $\phi_{1e}$, $A_{2e}$, $\phi_{2e}$                                   &	3183 &	3384.95  &	2.00 \\     
$A_{1f}$, $\phi_{1f}$, $A_{2f}$, $\phi_{2f}$                                   &	3183 &	3384.38  &	1.91 \\     
$A_{1N}$, $\phi_{1N}$, $A_{2N}$, $\phi_{2N}$                                   &	3183 &	3396.21  &	3.52 \\     
%$A_1$, $A_2$, $\Phi_1$, $\Phi_2$, $A_{1f}$, $\phi_{1f}$, $A_{2f}$, $\phi_{2f}$ &	3187 &	3392.28  &	2.12 \\     
\bottomrule
\end{tabular}
